A Memory Efficient Baseline for Open Domain Question Answering

Recently, retrieval systems based on dense representations have led to important improvements in open-domain question answering, and related tasks. While very effective, this approach is also memory intensive, as the dense vectors for the whole knowledge source need to be kept in memory. In this paper, we study how the memory footprint of dense retriever-reader systems can be reduced. We consider three strategies to reduce the index size: dimension reduction, vector quantization and passage filtering. We evaluate our approach on two question answering benchmarks: TriviaQA and NaturalQuestions, showing that it is possible to get competitive systems using less than 6Gb of memory.

==> introduction.tex <==
\section{Introduction}

Following the standard retriever-reader approach, open-domain question answering are commonly composed of two modules, the retriever and the reader.
Given an input question, the task of the retriever is to locate relevant documents in a knowledge source.
The core constraint faced by the retriever is to perform this retrieval step at the scale of large knowledge source such as Wikipedia.
Retrievers are specifically designed for this purpose: first each document of the knowledge source is embedded into a vector stored in an index.
Then given an input query, relevant documents are retrieved with a maximum inner product search in the pre-computed index using a library enabling to perform this operation efficiently such as FAISS~\citep{johnson2019billion}. 

The type of representation used to embed documents can be divided into two categories: sparse or dense.
Traditionally methods, such as TF-IDF or BM25~\citep{jones1972statistical, robertson1995okapi}, based on hand-crafted sparse features were used.
Sparse methods have only been outperformed by their dense counterparts very recently~\cite{karpukhin2020dense, guu2020realm}.
One of the feature distinguishing dense methods from sparse ones is that the document embeddings are learned using a neural network.

Both types of methods, sparse or dense, generally induce a large memory footprint to store the pre-computed indexes. 
This makes them difficult to use in memory constraint environment and impossible to communicate. 
This last point has been the focus of the EfficientQA competition recently organised at NeurIPS where evaluated system images were submitted to size constraints.

In this study we analyse how the performance of an unrestricted system achieving state-of-the-art performance degrades as more constraints on the size of the index and the data are applied. We show that it is possible to obtain systems of a reasonable size with a minimal performance loss.
